Asymptotic analysis of the sojourn time of a batch in an $M^{[X]}/M/1$ Processor Sharing Queue

In this paper, we exploit results obtained in an earlier study for the Laplace transform of the sojourn time $\Omega$ of an entire batch in the $M^{[X]}/M/1$ Processor Sharing (PS) queue in order to derive the asymptotic behavior of the complementary probability distribution function of this random variable, namely the behavior of $P(\Omega>x)$ when $x$ tends to infinity. We precisely show that up to a multiplying factor, the behavior of $P(\Omega>x)$ for large $x$ is of the same order of magnitude as $P(\omega>x)$, where $\omega$ is the sojourn time of an arbitrary job is the system. From a practical point of view, this means that if a system has to be dimensioned to guarantee processing time for jobs then the system can also guarantee processing times for entire batches by introducing a marginal amount of processing capacity.

==> data_matlab.tex <==
row= q x10;
col=rho* x 10
N=1M

meanW =

         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    2.8491    3.3163    4.0126         0         0    9.9698         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    7.1579    8.2916   10.0019         0         0   25.0974         0
         0         0   14.1056   16.5664   20.5566         0         0   50.7872         0

>> meanWb

meanWb =

         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    3.0543    3.6623    4.5951         0         0   13.3088         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    8.1252    9.9280   12.7173         0         0   42.1318         0
         0         0   16.3858   20.4420   27.2760         0         0   93.0302         
         
N=10M
meanWb =

         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    3.0678    3.6825    4.5745         0         0   13.3884         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    8.1453    9.9327   12.7583         0         0   41.7556         0
         0         0   16.6219   20.5796   26.5404         0         0   91.6515         0


meanW =

         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    2.8592    3.3325    4.0011         0         0   10.0135         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    7.1737    8.3009   10.0274         0         0   24.8916         0
         0         0   14.3206   16.6684   20.0237         0         0   50.0389         0


mean job &	mean batch& $q$	&$\rho^*$\\ \hline
2.8491 &	3.0543&	0.3&	0.5 \\
3.3163 &3.6623	& 	0.4& 	0.5 \\
4.0126 & 4.5951	 &	0.5	& 0.5 \\
9.9698 &	 13.3088	 & 0.8 &	0.5\\
\hline
7.1579 &	8.1252 &	0.3 &	0.8 \\
8.2916 &	9.9280 & 	0.4& 	0.8 \\
10.0019 &	12.7173 &	0.5	& 0.8 \\
25.0974 &	42.1318	 & 0.8 &	0.8 \\
\hline
 14.1056 &16.3858	&	0.3&	0.9 \\
16.5664 &20.4420	& 	0.4& 	0.9 \\
20.5566 &	27.2760 &	0.5	& 0.9 \\
50.7872 &	93.0302	 & 0.8 &	0.9 \\




N=70000

\begin{table}[hbtp]
\begin{tabular}{cccc} 
\hline
mean job &	mean batch& $q$	&$\rho^*$\\ \hline
2.8641 &	3.0707&	0,3&	0,5 \\
3.3635 &3.7137	& 	0,4& 	0,5 \\
3.9842 & 4.5563	 &	0,5	& 0,5 \\
10.1701 &	13.6023	 & 0,8 &	0,5\\
\hline
7.1308 &	8.3970 &	0.3 &	0.8 \\
8.3121 &	10.406 & 	0.4& 	0.8 \\
9.9831 &	13.3529 &	0.5	& 0.8 \\
24.9948 &	41.9611	 & 0.8 &	0.8 \\
\hline
13.1535 &15.2586	&	0,3&	0,9 \\
15.6862 &19.3887	& 	0,4& 	0,9 \\
20.3515 &	26.9405 &	0,5	& 0,9 \\
62.8132 &	116.5948	 & 0,8 &	0,9 \\
\hline
\end{tabular}
\end{table}





